Robust Parameter Learning for Uncertain MDPs

Learning-based approaches to verifying unknown Markov decision processes (MDPs) often employ uncertain MDPs. These models use, for example, confidence intervals to capture transition uncertainty and allow synthesis of policies that are robust to this uncertainty. However, this approach typically quantifies uncertainty independently for individual transition probabilities, ignoring dependencies due to shared latent quantities. We propose to learn such models using parametric MDPs (pMDPs), where transition probabilities are expressions over a set of parameters. We project statistical uncertainty from empirical transition frequencies onto the pMDP's parameter space, yielding a probably approximately correct (PAC) uncertainty model for the underlying MDP that respects the algebraic dependencies between transitions. The resulting models are algorithmically challenging to solve, so we propose a hierarchy of sound polytopic outer approximations of the induced confidence set. We implement and evaluate our approach, demonstrating substantially tighter uncertainty estimates than classical interval-based uncertain MDP learning techniques.

==> tables/stats_table.tex <==
% Requires \usepackage{booktabs,multirow,array}
\begin{table}[t]
\centering
\caption{Salient characteristics of the considered benchmark instances. The last column indicates the property type: $\mathbb{P}$ denotes a temporal-logic satisfaction probability, while $\mathbb{E}$ denotes an expected-reward property.}
\vspace{5pt}
\setlength{\tabcolsep}{4pt}
\footnotesize
\renewcommand{\arraystretch}{0.95}
\resizebox{0.7\textwidth}{!}{%
\begin{tabular}{>{\centering\arraybackslash}m{3.3cm} >{\centering\arraybackslash}m{2cm} >{\centering\arraybackslash}m{1.4cm} >{\centering\arraybackslash}m{1.55cm} >{\centering\arraybackslash}m{1.2cm} >{\centering\arraybackslash}m{1.2cm} >{\centering\arraybackslash}m{1.2cm}}
\toprule
\textbf{Benchmark} & \textbf{Instance} & \textbf{$\mathbf{|S|}$} & \textbf{$\mathbf{|T|}$} & \textbf{$\mathbf{|\Theta|}$} & \textbf{$\mathbf{|\Lambda|}$} & \textbf{Prop.} \\
\midrule
\multirow[c]{3}{*}{Aircraft} & (50, 10) & 5463 & 73033 & 6 & 721 & $\mathbb{P}$ \\
 & (100, 20) & 39028 & 551598 & 6 & 1441 & $\mathbb{P}$ \\
 & (200, 40) & 294458 & 4285228 & 6 & 2881 & $\mathbb{P}$ \\
\addlinespace[2pt]
\multirow[c]{3}{*}{Betting Game} & (50) & 13500 & 111678 & 2 & 2613 & $\mathbb{E}$ \\
 & (100) & 52000 & 448378 & 2 & 5283 & $\mathbb{E}$ \\
 & (150) & 100800 & 879738 & 2 & 7413 & $\mathbb{E}$ \\
\addlinespace[2pt]
\multirow[c]{3}{*}{Engagement} & (100) & 1994 & 5962 & 5 & 61 & $\mathbb{E}$ \\
 & (300) & 5994 & 17962 & 5 & 61 & $\mathbb{E}$ \\
 & (1000) & 19994 & 59962 & 5 & 61 & $\mathbb{E}$ \\
 \addlinespace[2pt]
\multirow[c]{3}{*}{Mars Rover} & (50, 50) & 191868 & 1003861 & 6 & 643 & $\mathbb{P}$ \\
 & (75, 75) & 550447 & 2973287 & 6 & 943 & $\mathbb{P}$ \\
 & (125, 125) & 1749083 & 9591771 & 6 & 1543 & $\mathbb{P}$ \\
\addlinespace[2pt]
\multirow[c]{3}{*}{Glider} & (21, 17) & 357 & 5209 & 4 & 777 & $\mathbb{E}$ \\
 & (51, 47) & 2397 & 37059 & 4 & 4977 & $\mathbb{E}$ \\
 & (106, 99) & 4623 & 72183 & 4 & 9504 & $\mathbb{E}$ \\
\addlinespace[2pt]
 \multirow[c]{3}{*}{Parallel Betting} & (5) & 3051 & 15543 & 3 & 477 & $\mathbb{E}$ \\
 & (10) & 21006 & 187730 & 3 & 1077 & $\mathbb{E}$ \\
 & (20) & 151556 & 1846840 & 3 & 185209 & $\mathbb{E}$ \\
\bottomrule
\end{tabular}
} % end of resizebox
\label{tab:stats_same_suite}
\vspace{-5pt}
\end{table}
\renewcommand{\arraystretch}{1}

==> text/overview.tex <==
\label{sec:overview}
We extend the discussion from Section~\ref{sec:intro} with an illustrative example that captures the main idea of our approach. Figure~\ref{fig:gridworld_left} shows a Mars-rover navigation domain, inspired by the semi-autonomous vehicle environment in~\cite{DBLP:conf/tacas/Junges0DTK16,DBLP:journals/jfr/StucklerSSTB16}.
\vspace{-15pt}
\input{figures/example}
\vspace{-3pt}
A~controller communicates with the rover via two satellites, each inducing a lossy communication channel: messages may fail to be delivered with some probability. The rover’s objective is to collect rock samples and return to its home position.

The probability of communication loss depends on the rover’s position. This positional dependence is known and proportional to the distance to each satellite, while the reliabilities of the two channels are unknown. The probability of successful communication, and hence of executing intended moves, is a function of the unknown reliability parameters. At each position it has the form
\[
v^\top \theta \;=\; v_1\theta_1 + v_2\theta_2,
\]
where the coefficients $v=(v_1,v_2)$ are determined by the current position and $\theta=(\theta_1,\theta_2)$ are the unknown satellite reliabilities. The domain can thus be modelled as a pMDP, with symbolic probability expressions as shown in Figure~\ref{fig:var2_mdp_right}.

The goal is to synthesise a controller policy that maximises the probability that the rover successfully completes its task under communication uncertainty. Since the exact transition probabilities are unknown, we want to learn from sampled interactions with the rover. A standard approach is to construct from these samples an IMDP, i.e., an MDP in which transition probabilities are not fixed but constrained to intervals of valid probabilities. Given an IMDP, we can synthesise a policy that is robust against the worst-case transition probabilities within the intervals. If the learned intervals come with formal confidence guarantees on inclusion of the true transition probability, this yields a certified lower bound on the probability that the rover completes its task under the robust policy.


\input{figures/coordinate_2}

IMDP learning derives, for each unknown transition probability, a confidence interval from the observed samples, as depicted in Figure~\ref{fig:threepanel_param_b}. This inherently treats the unknown transition probabilities as \emph{independent} and learns them as separate intervals. In the rover domain, however, transition probabilities are not independent: they arise from parametric expressions over a shared underlying parameter instantiation for $\theta$. Our approach leverages these dependencies by projecting the learned per-probability intervals through the parametric structure into the parameter space. Since the expressions are linear in this example, a learned interval $[l,u]$ yields two linear constraints of the form
\[
l \leq v_1\theta_1 + v_2\theta_2 \leq u
\]
for each expression in the pMDP. Hence, the projection induces a polytope $\mathcal{U}$ of plausible parameter instantiations $\uu$, as shown in Figure~\ref{fig:threepanel_polytope}. This polytope inherits the confidence guarantees of the original per-probability uncertainty sets: with high confidence, the true (unknown) parameter instantiation lies in $\mathcal{U}$.

Together with the parametric structure of the underlying pMDP, the uncertainty region $\mathcal{U}$ induces a UMDP that is tighter than the one obtained from the per-probability intervals alone, as it exploits the parametric information to rule out distributions that are inconsistent with $\mathcal{U}$. Solving the resulting UMDP therefore yields less conservative robust policies and tighter high-confidence performance guarantees from the same data. A further advantage is that the rover does not necessarily need to visit high-risk regions in order to reduce uncertainty there. Information about the unknown parameters propagates through the model, so collecting data in lower-risk regions can reduce the uncertainty also for regions that have not been explored. This comes without loss of generality: when the pMDP exhibits no exploitable structure, each transition probability is an independent parameter and we recover the standard UMDP learning~setting.

